The Colorful Future of LLMs: Evaluating and Improving LLMs as Emotional Supporters for Queer Youth

Queer youth face increased mental health risks, such as depression, anxiety, and suicidal ideation. Hindered by negative stigma, they often avoid seeking help and rely on online resources, which may provide incompatible information. Although access to a supportive environment and reliable information is invaluable, many queer youth worldwide have no access to such support. However, this could soon change due to the rapid adoption of Large Language Models (LLMs) such as ChatGPT. This paper aims to comprehensively explore the potential of LLMs to revolutionize emotional support for queers. To this end, we conduct a qualitative and quantitative analysis of LLM's interactions with queer-related content. To evaluate response quality, we develop a novel ten-question scale that is inspired by psychological standards and expert input. We apply this scale to score several LLMs and human comments to posts where queer youth seek advice and share experiences. We find that LLM responses are supportive and inclusive, outscoring humans. However, they tend to be generic, not empathetic enough, and lack personalization, resulting in nonreliable and potentially harmful advice. We discuss these challenges, demonstrate that a dedicated prompt can improve the performance, and propose a blueprint of an LLM-supporter that actively (but sensitively) seeks user context to provide personalized, empathetic, and reliable responses. Our annotated dataset is available for further research.

==> 9.acknowledgement.tex <==
\section{Acknowledgement}
\label{sec:acknowledgement}
We express our gratitude to "Hoshen," the educational and advocacy organization representing the LGBTQ+ community in Israel, for sharing their valuable knowledge with us. Especially to Mor Nahari (CEO), Adi Lev (Northern Region Coordinator), and Yaron Avtalion.

Moreover, we would like to thank Anat Bar, Ilanit Sobol, Itay Nakash, Maya Zadok, Mor Ventura, Natalie A. Philip, Roi Gabay, Rotem Dror, Sapir Varshevski for their valuable contributions to our research.

==> figures/alert_tex.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1\textwidth]{figures/2.pdf}
    \caption{efe}
    \label{fig:alert}
\end{figure*}

==> figures/chat_orthodox1_tex_old.tex <==
\begin{figure*}[h]
     \centering
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example1.pdf}
         \caption{}
         \label{fig:example1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example2.pdf}
         \caption{}
         \label{fig:example2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.8\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/example3.pdf}
         \caption{}
         \label{fig:example3}
     \end{subfigure}
    \caption{Our main case study (\S\ref{sub:current}), which is based on a conversation between a queer, ultra-orthodox teenager, and ChatGPT. The personal information is added in a \textbf{sequential order}: First, the writer identifies only as a female and asks about how acceptable is to be attracted to women. In response, the generated answer affirms, ``Absolutely!'' and emphasizes that ``Same-sex attraction is a natural and normal variation of human sexuality, and there is nothing wrong or abnormal about it.'' Ultimately, it encourages to ``Embrace your identity and be proud of who you are.''. 
    Upon introducing the context of being a teenager, the revised answer now reflects a greater degree of uncertainty concerning the writer's sexual orientation. Furthermore, it acknowledges that ``Sexual orientation can be fluid, and it's okay if your feelings evolve or change over time.'' The response also encourages to seek support and open up about their experiences once they feel comfortable. Ultimately, concludes that it is important to ``Trust yourself and remember that you deserve love and respect, regardless of your sexual orientation.''.
    When the ultra-orthodox background was added, chatGPT acknowledged the unique challenges faced: ``If you're an ultra-orthodox teenager and exploring your sexual orientation, it can be particularly challenging due to the religious and cultural context''. And It highlights several suggestions, The response concludes by emphasizing that ``your journey is unique, and it's important to prioritize your well-being and emotional health throughout the process.''. \textbf{The chatGPT conversation of this figure continues in Figure~\ref{fig:orthodox2}}}
    \label{fig:orthodox}
\end{figure*}

==> figures/chat_orthodox2_tex_old.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/example2.pdf}
    \caption{The continuation of the conversation from Figure~\ref{fig:orthodox}.}
    \label{fig:orthodox2}
\end{figure*}

==> figures/chat_orthodox_separate_tex.tex <==
\begin{figure*}[h]
\centering
\begin{subfigure}[b]{0.98\textwidth}
\centering
   \includegraphics[width=0.7\linewidth]{figures/1.pdf}
   \caption{}
   \label{fig:1} 
\end{subfigure}

\begin{subfigure}[b]{0.98\textwidth}
\centering
   \includegraphics[width=0.7\linewidth]{figures/2.pdf}
   \caption{}
   \label{fig:2}
\end{subfigure}

\begin{subfigure}[b]{0.98\textwidth}
\centering
   \includegraphics[width=0.7\linewidth]{figures/3.pdf}
   \caption{}
   \label{fig:3}
\end{subfigure}

\caption{The main case study based on ChatGPT conversation with added information in \textbf{new chat session approach} \textbf{(a)} Example of a response by ChatGPT where the writer identifies as female and inquires about the acceptability of being attracted to women. In response, the generated answer affirms, ``Absolutely!'' and emphasizes that ``Same-sex attraction is a natural and normal variation of human sexuality, and there is nothing wrong or abnormal about it.'' Ultimately, it encourages to ``Embrace your identity and be proud of who you are.''; \textbf{(b)} After providing an additional context, that being a teenager, the chatGPT raised a content violation alert and stopped generating; \textbf{(c)} when adding the context of being ultra-orthodox in a new chat session, the only discernible difference from the original answer (i.e., without the additional information) is the inclusion of an extra paragraph. This paragraph acknowledges that ``Different cultures and religious beliefs may have varying perspectives on sexuality, including same-sex attraction.''}
\label{fig:orthodox_separate}
\end{figure*}


==> figures/grid_tex.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/grid.pdf}
    \caption{Our scheme for categorizing AI sexual supporters based on two key dimensions: reliability (horizontal) and personalization (vertical). The reliability dimension evaluates the system's reliance on expert opinions and credible information. The personalization dimension assesses the ability to offer tailored support through user identification and response adaptation.}
    \label{fig:grid}
\end{figure}
